Sublinear quantum algorithms for estimating von Neumann entropy

Entropy is a fundamental property of both classical and quantum systems, spanning myriad theoretical and practical applications in physics and computer science. We study the problem of obtaining estimates to within a multiplicative factor $\gamma>1$ of the Shannon entropy of probability distributions and the von Neumann entropy of mixed quantum states. Our main results are: $\quad\bullet$ an $\widetilde{\mathcal{O}}\left( n^{\frac{1+\eta}{2\gamma^2}}\right)$-query quantum algorithm that outputs a $\gamma$-multiplicative approximation of the Shannon entropy $H(\mathbf{p})$ of a classical probability distribution $\mathbf{p} = (p_1,\ldots,p_n)$; $\quad\bullet$ an $\widetilde{\mathcal{O}}\left( n^{\frac12+\frac{1+\eta}{2\gamma^2}}\right)$-query quantum algorithm that outputs a $\gamma$-multiplicative approximation of the von Neumann entropy $S(\rho)$ of a density matrix $\rho\in\mathbb{C}^{n\times n}$. In both cases, the input is assumed to have entropy bounded away from zero by a quantity determined by the parameter $\eta>0$, since, as we prove, no polynomial query algorithm can multiplicatively approximate the entropy of distributions with arbitrarily low entropy. In addition, we provide $\Omega\left(n^{\frac{1}{3\gamma^2}}\right)$ lower bounds on the query complexity of $\gamma$-multiplicative estimation of Shannon and von Neumann entropies. We work with the quantum purified query access model, which can handle both classical probability distributions and mixed quantum states, and is the most general input model considered in the literature.

==> quant-prelims.tex <==

% The usual unit of classical computation is the bit, a Boolean variable taking values in $\mathbb{Z}_2=\{0,1\}$. Its analogue in quantum computation is called the qubit, and represents the state of a physical quantum $2$-level system. A qubit can take values or \emph{states} in $\C^2$, i.e.\ linear combinations or superpositions of two classical values (complex numbers)
% \[
% \alpha\ket0 + \beta\ket1
% \] In particular we require that $|\alpha|^2+|\beta|^2=1$. We have also introduced the Dirac bra-ket in the above: 
% \[
% \ket0 := \begin{pmatrix}1\\0\end{pmatrix},~~~~~\ket1 := \begin{pmatrix}0\\1\end{pmatrix}.
% \]
% More generally, the set of states an $m$-qubit quantum register can take is the set of unit vectors
% \begin{equation*}
% \label{eq:quantum-state}
% \ket\psi = \sum_{i\in\{0,1\}^m}\alpha_i\ket i\text{ with } \alpha_i\in\C,\text{ such that }\sum_i|\alpha_i|^2=1
% \end{equation*}
% in the Hilbert space spanned by a set of orthonormal basis vectors $\{\ket i, i\in\{0,1\}^m\}$, known as the \emph{computational basis}. Such an $m$-qubit state is said to be a superposition of the $m$ basis states. Each $\alpha_i$ is called the \emph{amplitude of basis state $\ket i$}, and the $L_2$ normalisation condition on $\ket{\psi}$ will enable us to treat the $\{|\alpha_i|^2\}$ as probabilities. We interpret the vector $\ket i$ as the $m$-dimensional complex vector $v_i$ with entries given by $(v_i)_j=\delta_{ij}$, and also interchangeably as the integer $i$ or the bit string that gives its binary representation $b_1\ldots b_m$ where $b_i$ is either $0$ or $1$. Furthermore, and of key importance to quantum mechanics and computation, the vector $\ket{b_1\ldots b_m}\in\C^{2^m}={(\C^2)}^{\otimes m}$ is interpreted as a tensor product 
% \[\ket{b_1\ldots b_m}=\ket{b_1}\otimes\ket{b_2}\otimes\ldots\otimes\ket{b_m}\]
% of the $m$ vectors $\ket{b_i}$ in $\C^2$. The $\otimes$ is often dropped for convenience, and we write $\ket{b_1}\ket{b_2}$ for $\ket{b_1}\otimes\ket{b_2}$. 

The conjugate transpose of a column vector $\ket{\psi}$ is a row vector denoted by $\bra{\psi}$. The conjugate transpose and the transpose of an operator $A$ are denoted by $A^\dag$ and  $A^\mathrm{T}$, respectively.
The inner product of $\ket{\psi}$ and $\ket{\phi}$ is denoted by $\braket{\psi|\phi}$, while their outer product $\ketbra{\psi}{\phi}$ is a matrix. We will also occasionally denote rank-1 projectors by a capitalised Pi, e.g.\ $\Pi_\psi:=\ketbra{\psi}{\psi}$. 



Physically, the computational basis states that we usually choose correspond to eigenstates of the $z$-component of the spin operator (i.e.\ the Pauli Z operator) of the underlying system. In addition to normalisation, quantum states also have a `global phase invariance', in that for any $\theta\in\R$, $\ket{\psi}$ is identified with $\ee^{\ii \theta}\ket{\psi}$. 


 

% \noindent\textbf{Unitary operators}: There are two ways in which we can compute on a state $\ket{\psi}$. The first is by \emph{unitary evolution} of the system under the Schr\"odinger equation with a specified Hamiltonian operator $H$
% \[
% i\frac{d\ket\psi}{dt} = H\ket\psi,
% \]
% where $H$ is a hermitian matrix. Closed systems undergo reversible dynamics in quantum mechanics, and this dynamics is represented by unitary matrices. Since we can think of $\ket\psi$ as a vector in $\C^{2^m}$, a computation is represented by multiplication of this state by a $U\in\text{SU}(2^m)$, i.e. $\ket{\psi_{\text{out}}}=U\ket{\psi_{\text{in}}}$. 

Recall that a matrix $U$ is said to be unitary if $UU^{\dagger}=\id$, where $U^{\dagger}$ is the conjugate transpose of $U$. Unitary operators then act by left multiplication on pure states vector, and by conjugation on density matrices. 

\noindent\textbf{Measurements}: The second kind of operation we can perform on $\ket\psi$ is measurement. For our purposes, the postulates of quantum mechanics say that on measuring a superposition state $\ket\psi$ as above \emph{in the basis $\{\ket i\}$}, we obtain as outcome the random $m$-bit string corresponding to the basis state $\ket i$ with probability $p(i)=|\alpha_i|^2$. Since we have chosen states to be normalised, the measurement gives a valid probability mass function over the set of classical $m$-bit strings. After the measurement, the state ``collapses'' to the observed basis state $\ket{i}$, and no further information can be retrieved from the original state;  to repeat the sampling achieved by this measurement, we need to prepare $\ket{\psi}$ for each repetition. 

% Thus a \emph{measurement} on an $m$-qubit state $\ket{\psi}$ in the computational basis is a sampling process that returns a randomly chosen $m$-bit string $x$ with probability $p(x)=|\alpha_x|^2$. 

For two registers $A$ and $B$ and their state $\ket{\psi}^{AB}=\sum_{x,x}\alpha_{x,x'}\ket{x}^A\otimes\ket{x'}^B$, a measurement of the register $B$ for $\ket{\psi}^{AB}$ in the computational basis $\{\ket{x'}^B\}$ of system $B$ yields an outcome $x'$ with probability $p(x')=\sum_{x}p(x,x')$, where $p(x,x')={|\alpha_{x,x'}|}^2$.
The superscripts of a state or an operator represent which register the state or the operator belongs to; we omit the superscript if it is clear from the context.


%----------------------------------------------------------
\noindent\textbf{Input models}: The quantum analogue of the classical query model, where inputs are accessed via a black-box or oracle that can be queried with an index $i$ and returns the $i$-th bit of the input bit string is defined as follows. For a bit string $x\in\{0,1\}^n$ we assume access to a unitary $\O_x$ which performs the map
\begin{equation*}
    \O_x\ket i\ket b \ket z = \ket i \ket{b\oplus x_i} \ket{z},
\end{equation*}
where the first register consists of $\lceil\log n\rceil$ qubits, the second is a single qubit register to store the output of the query, and the third is any additional workspace the quantum computer might have and is not affected by the query. Here $\oplus$ is addition on $\mathbb{Z}_2$, i.e.\ the $\cc{XOR}$ operation in Boolean logic. Note that $\O_x$ can be used by a quantum computer to make queries in superposition:
\begin{equation*}
    \O_x\left(\frac1n\sum_{i=1}^n\ket i\ket b \ket z\right) = \frac1n\sum_i\ket i \ket{b\oplus x_i} \ket{z},
\end{equation*}


\parahead{Quantum algorithms :} 
% Broadly speaking, a quantum algorithm starts by initializing $m$ qubits in a fixed state $\ket{0}^{\otimes m}$, which we may write as $\ket{0}$ if $m$ is clear from context.
% Then, we apply a $2^m$-dimensional unitary operator $U$ to $\ket{0}^{\otimes m}$, to prepare a state $U\ket{0}^{\otimes m}$.
% Finally, a measurement on $U\ket{0}^{\otimes m}$ is performed to sample an $m$-bit string from the probability distribution given by $U\ket{0}^{\otimes m}$.

As in classical computer science, we can work in a quantum circuit model, by first fixing a basic set of operations or `gates' (analogous to classical Boolean {\small AND} and {\small OR}), achievable on the underlying hardware. It is then possible to compile a large `algorithm' $U$ down into elementary unitary operations, or quantum gates, and represent it by a quantum circuit composed of sequential applications of unitaries acting on at most two qubits at a time. Each of these unitaries is called an elementary quantum gate, and we can choose to work with different basic or fundamental `gate sets' that can be used to construct an approximate circuit for any unitary, to any arbitrary precision, via the Solovay-Kitaev theorem. The runtime of a quantum algorithm is essentially determined by the number of elementary quantum gates in its circuit. Given a circuit for a unitary, it is straightforward to implement its inverse, or control its application on ancillary registers, with only a small overhead in the gate complexity.



%----------------------------------------------------------
\noindent\textbf{Complexity measures}: For many theoretical studies in complexity, the query input model is a powerful setting where several results have been proven. In this model, the total number of queries made to the input oracle is the primary measure of algorithmic complexity, known as the \emph{query complexity}. 

For practical purposes, it is more important to understand the number of elementary quantum gates used to implement the unitary circuit corresponding to the algorithm in the quantum circuit model. This is known as the \emph{gate complexity} of the algorithm. The depth of the circuit is directly related to the time complexity, and gives an idea of how parallelisable the algorithm is.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





==> scratch-shannon-log-approx.tex <==
\section{Estimating Shannon entropy to multiplicative precision using purified quantum samples}
Consider the following function for some $\alpha\in(0,1)$ 
\begin{equation}
    f_\alpha(x) \defeq \frac{1}{2\alpha}\left(x^{\alpha}-x^{-\alpha}\right)
\end{equation}
on a domain $(\beta, 1]$ for some $\beta>0$. We have the series expansions \comment{check radius of convergence, point about which you're expanding}
\begin{align}
    x^{\pm\alpha} &= e^{\pm\alpha\log x} \nonumber\\
            &= 1 \pm\alpha\log x + \frac{(\alpha\log x)^2}{2!} \pm\frac{(\alpha\log x)^3}{3!} + \ldots     
\end{align}
and so
\begin{equation}
    f_\alpha(x) = \log x\cdot\left(1 + \frac{(\alpha\log x)^2}{3!} +\frac{(\alpha\log x)^4}{5!} + \ldots\right)
\end{equation}
Our goal is for $f_\alpha(x)$ to be a good approximation for $\log x$ on $(\beta,1]$. We have an error given by
\begin{align}
    r(\alpha,x)=\Abs{\frac{\log x - f_\alpha(x)}{\log x}}\nonumber\\ 
        &= \sum_{j=1}^\infty\frac{(\alpha\log x)^{2j}}{(2j+1)!}.
\end{align}
We want this tail series to be small for every $x\in(\beta,1]$. Notice that if $\Abs{\alpha\log\beta}<1$, the series always converges and we have
\begin{equation}
    r(\alpha,x) \leq \frac{1}{6}\cdot\frac{(\alpha\log x)^2}{1-(\alpha\log x)^2}. 
\end{equation}
Requiring that $\forall x\in(\beta,1]$, $r(\alpha,x)$ be smaller than some $\epsilon\in(0,1)$ we have
\begin{equation}
    \frac{1}{6\epsilon} \leq  \frac{1}{(\alpha\log x)^2} - 1,
\end{equation}
and so
\begin{equation}
    \alpha \leq \frac{1}{|\log\beta|}\cdot\sqrt\frac{6\epsilon}{1+6\epsilon}.
\end{equation}
Importantly, notice that 
\[
    \alpha = \O\left(\frac{\sqrt{\epsilon}}{\log\nicefrac{1}{\beta}}\right).
\]
Thus we have a $\epsilon$-multiplicative approximation of the logarithm for $x\in(\beta,1]$, i.e.\
\begin{equation}
    \label{eq:mult-approx-log}
    \Abs{\frac{\log x - f_\alpha(x)}{\log x}} \leq \epsilon.
\end{equation}

Recall that the Shannon entropy is defined by \cref{eq:shannon_entropy}
\[
    H(\pbold) = -\sum_i p_i\log p_i.
\]
We will first divide the domain into two sets: $B_\beta=\{i\in [n] : p_i\geq \beta\}$, and $S_{\beta}=[n]\setminus B_{\beta}$. Notice that $H(\pbold)=H_{B_{\beta}}(\pbold)+H_{S_{\beta}}(\pbold)$ \comment{define this notation properly in the prelims}.

For $i\in B_\beta$, if we replace the logarithm above with the function $f_\alpha$, we can calculate the error incurred by $H_{B_{\beta}}(\pbold)$ as follows. Observe that \cref{eq:mult-approx-log} implies that $\forall x\in(\beta, 1]$
\begin{equation}
    -\epsilon\log x \leq \log x - f_\alpha(x) \leq \epsilon\log x.
\end{equation}
Applying this to the case of the entropy of $\pbold$ and summing over $p_i$ for $i\in B_\beta$, we have
\begin{equation}
    -\epsilon\cdot\sum_{i\in B_{\beta}} p_i \log p_i \leq \sum_{i\in B_{\beta}} p_i\log p_i - \sum_{i\in B_{\beta}} p_if_\alpha(p_i) \leq \epsilon\cdot\sum_{i\in B_{\beta}} p_i \log p_i
\end{equation}
and so, noticing that the signs flip due to the negative sign in the definition of $H$, we have
\begin{equation}
    \epsilon H_{B_{\beta}}(\pbold) \geq -H_{B_{\beta}}(\pbold) - \sum_{i\in B_{\beta}} p_i f_\alpha(p_i) \geq -\epsilon\sum_{i\in B_{\beta}} p_if_\alpha(p_i),
\end{equation}
which means that $-\sum_i p_i f_\alpha(p_i)$ is a multiplicative approximation to the entropy, i.e.\
\begin{equation}
    \label{eq:mult-error-H-f}
    \Abs{H_{B_{\beta}}(\pbold)-\left(-\sum_{i\in B_{\beta}} p_i f_\alpha(p_i)\right)} \leq \epsilon\cdot H_{B_{\beta}}(\pbold).
\end{equation}

Our goal will be to prepare a state that has squared amplitude equal to $H(\pbold)$ on part of it flagged by $\ket{0}$ in the ancilla. One way to do this is to prepare a state that looks like
\[
    \sum_i \sqrt{p_i} \sqrt{\log p_i} \ket{\psi_i}\ket{i}\ket{0} + \ket{\text{junk}}\ket{1}.
\]
Since we cannot get $H(\pbold)$ itself, we approximate it with 
\[
    \tilde{H}(\pbold) \defeq \sum_i p_i f_\alpha(p_i),
\]
and for this we will need a state that looks like
\[
    \sum_i \sqrt{p_i} \sqrt{f_\alpha(p_i)} \ket{\psi_i}\ket{i}\ket{0} + \ket{\text{junk}}\ket{1}.
\]
Thus we need to apply the quantum singular value transformation corresponding to the function $\sqrt{f_\alpha(x)}$. Note that the square root $\sqrt{f_\alpha(x)}$ is a good multiplicative approximation for $\sqrt{\log x}$, since
\begin{align*}
    \Abs{\frac{\sqrt{a(x)}-\sqrt{b(x)}}{\sqrt{a(x)}}\cdot \frac{\sqrt{a(x)}+\sqrt{b(x)}}{\sqrt{a(x)}}} = \Abs{\frac{a(x)-b(x)}{a(x)}} &\leq \epsilon \\
        \implies \Abs{\frac{\sqrt{a(x)}-\sqrt{b(x)}}{\sqrt{a(x)}}} &\leq \epsilon
\end{align*}
since if $a(x)$ and $b(x)$ are positive,
\[
    \Abs{\frac{\sqrt{a(x)}+\sqrt{b(x)}}{\sqrt{a(x)}}} > 1.
\]

On the other hand, we cannot implement $\sqrt{f_\alpha(x)}$ or exactly, but only approximate it with a suitable polynomial. Suppose we have a polynomial $P(x)$ on the domain $(\beta, 1-\beta)$ such that $\forall x\in(\beta,1-\beta)$,
\begin{equation}
    \label{eq:poly-for-f-alpha}
    \Abs{\sqrt{f_\alpha(x)}-P(x)} < \epsilon_1,
\end{equation}
where the degree $d$ of $P(x)$ will be some function of $\beta$ and $\epsilon$ that will be of importance to us. Notice that we have
\begin{align}
\label{eq:f-to-p-square-to-log-error}
    \Abs{f_\alpha(x)-P^2(x)} &=\Abs{\left(\sqrt{f_\alpha(x)}-P(x)\right)\left(\sqrt{f_\alpha(x)}+P(x)\right)}\nonumber\\
        &\leq \epsilon_1\cdot\Abs{\left(\sqrt{f_\alpha(x)}+P(x)\right)}\nonumber\\
        &\leq 3\epsilon_1 \max_{x\in(\beta,1-\beta)} \sqrt{f_\alpha(x)}\nonumber\\
        &\leq 3\epsilon_1(1+\epsilon)\cdot\sqrt{\log\nicefrac{1}{\beta}}\nonumber\\
        &\leq 6\epsilon_1\cdot\sqrt{\log\nicefrac{1}{\beta}}.
\end{align}
So we set $\epsilon_1\to\epsilon/\sqrt{\log\nicefrac{1}{\beta}}$. Furthermore, \comment{insert modulus etc properly so that the logarithms are positive etc}
\begin{align}
    \Abs{\frac{\log x-P^2(x)}{\log x}} &= \Abs{\log x - f_\alpha(x) + f_\alpha(x) -P^2(x)}\nonumber\\
        &\leq \Abs{\frac{\log x - f_\alpha(x)}{\log x}} + \Abs{\frac{f_\alpha(x) - P^2(x)}{\log x}}\nonumber\\
        &\leq \epsilon + \displaystyle\frac{\epsilon_1}{\min_(\beta,1-\beta)\log x}\nonumber\\
        &\leq \epsilon + \frac{\epsilon_1}{\log(1-\beta)}\nonumber\\
        &\leq \epsilon + \frac{\epsilon_1}{\beta}
\end{align}
since $\log 1-x \geq -x$. This means we should also rescale $\epsilon_1\to\beta\epsilon$. Defining
\[
    \hat{H}(\pbold) \defeq \sum_i p_i \left(P(p_i)\right)^2,
\]
and recalling \cref{eq:mult-error-H-f}, we finally have that 
\begin{align}
    \Abs{\frac{H(\pbold)-\hat{H}(\pbold)}{H(\pbold)}} &\leq \Abs{\frac{H(\pbold)-\tilde{H}(\pbold)}{H(\pbold)}} + \Abs{\frac{\tilde{H}(\pbold)-\hat{H}(\pbold)}{H(\pbold)}}\nonumber\\
        &\leq \epsilon + \frac{\sum_i p_i\left(f_\alpha(p_i)-P^2(p_i)\right)}{\eta}\nonumber\\
        & \leq \epsilon + \frac{\epsilon_1\sum_i p_i}{\eta}\nonumber\\
        & \leq \epsilon  +\frac{\epsilon_1}{\eta},
\end{align}
where we assume $H(\pbold)\geq\eta>0$, which is reasonable because it is impossible to estimate a quantity to arbitrary multiplicative precision if it can be arbitrarily close to zero. Thus we will also need to rescale $\epsilon_1\to\eta\epsilon$. Together with \cref{eq:f-to-p-square-to-log-error} this indicates that we will have to choose 
\[
    \epsilon_1 = \O\left(\frac{\eta\beta\epsilon}{\log\frac{1}{\beta}}\right).
\]
\comment{Crucially, what will have to come to our rescue is the fact that using Taylor series approximations should give an exponential convergence in the degree of the approximating polynomial, i.e. the degree of the approximating polynomial only needs to grow as $\log\nicefrac{1}{\epsilon_1}$. This in addition to the fact that $\beta=n^{1/\gamma^2}$ should mean that the overhead introduced by the above error propagation should only be $\widetilde{\O}(\log n)$.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Creating block encodings or projected unitary encodings from the purified access oracle}
\citeauthor{Gilyen2018QuantumArithmetics} \cite{Gilyen2018QuantumArithmetics} give a series of lemmas showing how to implement block encodings of different kinds of inputs, of which we will be interested in the case of density operators. 

\begin{definition}[Definition 43, \cite{Gilyen2018QuantumArithmetics}]\label{defn:block-encoding}
    An $(\alpha, a, \epsilon)$ block encoding of an operator $A$ acting on $s$ qubits is a unitary $U$ acting on $a+s$ qubits, such that 
    \begin{equation}
        \norm{A - \alpha\Pi^\dagger U\Pi} \leq \epsilon,
    \end{equation}
    where the first register consists of ancillary qubits,  $\Pi:=\ket{0}^{\otimes a}\otimes\id_s$ is an isometry $\Pi:(\C^2)^{\otimes s}\mapsto\text{span}_{\C}\{\ket{0}^{\otimes a}\}\otimes (\C^2)^{\otimes s}$, and $\alpha,\epsilon\in(0,\infty)$.
\end{definition}

The conversion of a purified access oracle as in \cref{eq:purified-access-input-oracle} into a block encoding for $\rho$ can be achieved using the following result.  

\begin{lemma}[Lemma 45, \cite{Gilyen2018QuantumArithmetics}]
\label{lem:rho_block_encoding}
    Given a unitary $U_\rho$ acting on $a+s$-qubits, which prepares a purification $U_\rho\ket{0}\ket{0}=\ket{\rho}$ of an $s$-qubit density operator $\rho$, such that $\Tr[a]{\proj{\rho}}=\rho$, the unitary
    \begin{equation*}
        U=\left(U_\rho^\dagger\otimes\id_s\right)\left(\id_a\otimes \cc{SWAP}_s\right)\left(U_\rho\otimes\id_s\right)
    \end{equation*} gives an exact $(1, a+s, 0)$ block encoding of $\rho$.
\end{lemma}

This means that the unitary $U$ has the block form 
\begin{equation*}
    U = \begin{pmatrix}
            \rho & \cdot \\
            \cdot & \cdot
        \end{pmatrix},
\end{equation*}
where we have not specified the $a+s-1$ other $s$-qubit blocks on the diagonal.

In the special case when $\rho$ is diagonal in the computational basis and represents a classical probability distribution, a different technique for `projected unitary' encoding offers us access to the $\sqrt{p_i}$, in contrast to the above technique of block encoding which provides access to the $p_i$. 

First define the projection operators $\Pi=\id\otimes\proj{0}\otimes\proj{0}$ and $\tilde{\Pi}=\proj{0}\otimes\proj{0}\otimes\id$, where the third register contains the ancilla, and the first two contain states of the system. We also need a unitary map $W$ that prepares the maximally entangled state on the two copies of the system register: \[\ket{0}\ket0\longmapsto\frac1d\sum_{j=1}^d\ket j\ket j.\] 
With these operators and the purified access oracle $U_\rho$, we can define the unitary
\begin{equation*}
    U' = \left(\id\otimes U_\rho^{\dagger}\right)\left(W\otimes\id\right),
\end{equation*}
which gives rise to the following projected unitary encoding
\begin{equation*}
    \label{eq:gilyen_encoding}
    \Pi U'\tilde{\Pi} = \frac1d\sum_{j=1}^d\ketbra{\phi_j'}{0}\otimes\ketbra{0}{0}\otimes\ketbra{0}{\psi_j},
\end{equation*}
where $\{\ket{\phi_j'}\}$ is a Schmidt basis for the first half of the bipartite maximally entangled state.

This encoding has a leading normalisation factor of $\frac{1}{\sqrt{d}}$, which directly contributes a factor of $\sqrt d$ to the complexity of entropy estimation for quantum density matrices. It might be reasonable to ask if this factor be improved by using, e.g.\ an embezzling state of the form 
\[
\ket{\mu} := \mathcal{N}\sum_{j=1}^d \frac1j\ket j\ket j,
\]
where $\mathcal N = \sum_{j=1}^d\frac1j$ is the normalisation. What if we have coefficients $c_j$ instead of just $j$?

% proof of block encoding of density matrix

\begin{proof}
    % Let $r$ be the Schmidt rank $\rho\in\C^{d\times d}$ (where $d=2^s$), and let $\{\ket{\psi_k}:k=1,\ldots,d\}$ and $\{\ket{\phi_k}:k=1,\ldots,r\}$ be orthonormal bases for the system and purifying subspaces respectively. Taking $p=(p_1,\ldots,p_d)\in[0,1]^d$ such that
    As in \eqref{eq:purified-access-input-oracle}, we have (we will drop the $a$ and $d$ subscripts later for convenience)
    \begin{equation}
    U_\rho\ket{0}^{\otimes a+s} = \ket{\rho} = \sum_{i=1}^{d}\sqrt{p_i}\ket{\phi_i}_a\ket{\psi_i}_s,
    \end{equation}
    where the summation runs up to $d$ since the Schmidt rank of $\rho$ is at most $d$, and
    \[  
    \Tr[a]{\ketbra{\rho}{\rho}}=\sum_{i=1}^d p_i\proj{\psi_i}_d=\rho.
    \]
    To see that $U$ is indeed a block encoding of $\rho$, we can check the condition in the definition of block encodings given above; with $\Pi:=\ket{0}^{\otimes a+s}\otimes\id_d$ we have
    \begin{align*}
        \Pi^\dagger U\Pi &= \left(\bra{0}^{\otimes a+s}\otimes\id_s\right)\left(U_\rho^\dagger\otimes\id_s\right)\left(\id_a\otimes \cc{SWAP}_s\right)\left(U_\rho\otimes\id_s\right)\left(\ket{0}^{\otimes a+s}\otimes\id_s\right)\nonumber\\
            &=\left(\bra\rho\otimes\id_s\right)\left(\id_a\otimes \cc{SWAP}_s\right)\left(\ket\rho\otimes\id_s\right)\nonumber\\
            &=\left(\bra\rho\otimes\id_s\right)\left(\id_a\otimes \cc{SWAP}_s\right)\left(\sum_{i=1}^{d}\sqrt{p_i}\ket{\phi_i}_a\ket{\psi_i}_s\otimes\sum_{j=1}^d\proj{\psi_j}_s\right)\nonumber\\
            &=\left(\bra\rho\otimes\id_s\right)\left(\id_a\otimes \cc{SWAP}_s\right)\left(\sum_{i=1}^{d}\sum_{j=1}^d\sqrt{p_i}\ket{\phi_i}_a\ket{\psi_j}_s\otimes\ketbra{\psi_i}{\psi_j}_s\right)\nonumber\\
            &=\left(\sum_{k=1}^d\sqrt{p_k}\bra{\phi_k}_a\bra{\psi_k}_s\otimes\id_s\right)\left(\sum_{i=1}^{d}\sum_{j=1}^d\sqrt{p_i}\ket{\phi_i}_a\ket{\psi_j}_s\otimes\ketbra{\psi_i}{\psi_j}_s\right)\nonumber\\
            &=\sum_{i=1}^{d}\sum_{j=1}^d\sum_{k=1}^d\sqrt{p_i}\sqrt{p_k}\braket{\phi_k|\phi_i}_a\braket{\psi_k|\psi_j}_s\otimes\ketbra{\psi_i}{\psi_j}_s\nonumber\\
            &=\sum_{i=1}^d p_i\proj{\psi_i},
    \end{align*}
    where we've used the completeness relation $\id_s=\sum_{i=1}^d\proj{\psi_i}_s$.
\end{proof}

